Hadronic Final States in Deep Inelastic Scattering at HERA

Results on the analysis of the hadronic final state in neutral current deep inelastic scattering at HERA are presented; recent results on inclusive single particle distributions, particle correlations and event shapes are highlighted.

==> brook.5 <==
%%BeginDocument: corfig10.eps
80 dict begin
/s {stroke} def /l {lineto} def /m {moveto} def /t {translate} def
/sw {stringwidth} def /r {rotate} def /rl {roll}  def /R {repeat} def
/d {rlineto} def /rm {rmoveto} def /gr {grestore} def /f {eofill} def
/c {setrgbcolor} def /lw {setlinewidth} def /sd {setdash} def
/cl {closepath} def /sf {scalefont setfont} def /black {0 setgray} def
/box {m dup 0 exch d exch 0 d 0 exch neg d cl} def
/NC{systemdict begin initclip end}def/C{NC box clip newpath}def
/bl {box s} def /bf {box f} def /Y { 0 exch d} def /X { 0 d} def 
/mp {newpath /y exch def /x exch def} def
/side {[w .77 mul w .23 mul] .385 w mul sd w 0 l currentpoint t -144 r} def
/mr {mp x y w2 0 360 arc} def /m24 {mr s} def /m20 {mr f} def
/mb {mp x y w2 add m w2 neg 0 d 0 w neg d w 0 d 0 w d cl} def
/mt {mp x y w2 add m w2 neg w neg d w 0 d cl} def
/m21 {mb f} def /m25 {mb s} def /m22 {mt f} def /m26 {mt s} def
/m23 {mp x y w2 sub m w2 w d w neg 0 d cl f} def
/m27 {mp x y w2 add m w3 neg w2 neg d w3 w2 neg d w3  w2 d cl s} def
/m28 {mp x w2 sub y w2 sub w3 add m w3 0 d 0 w3 neg d w3 0 d 0 w3 d w3 0 d
 0 w3 d w3 neg 0 d 0 w3 d w3 neg 0 d
 0 w3 neg d w3 neg 0 d cl s } def
/m29 {mp gsave x w2 sub y w2 add w3 sub m currentpoint t
 4 {side} repeat cl fill gr} def
/m30 {mp gsave x w2 sub y w2 add w3 sub m currentpoint t
 5 {side} repeat s gr} def
/m31 {mp x y w2 sub m 0 w d x w2 sub y m w 0 d
 x w2 sub y w2 add m w w neg d x w2 sub y w2
 sub m w w d s} def
/m2 {mp x y w2 sub m 0 w d x w2 sub y m w 0 d s} def
/m5 {mp x w2 sub y w2 sub m w w d x w2 sub y w2 add m w w neg d s} def
/DP {/PT exch def gsave 47.2 47.2 scale PT 1  eq { 16 16 1 [ 16 0 0 16 neg 0 16
] { < AA AA 55 55 AA AA 55 55 AA AA 55 55 AA AA 55 55 AA AA 55 55 AA AA 55 55
AA AA 55 55 AA AA 55 55 > } image } if PT 2 eq { 16 16 1 [ 16 0 0 16 neg 0 16
] { < BB BB EE EE BB BB EE EE BB BB EE EE BB BB EE EE BB BB EE EE BB BB EE EE
BB BB EE EE BB BB EE EE > } image } if PT 3 eq { 16 16 1 [ 16 0 0 16 neg 0 16
] { < FF FF BB BB FF FF EE EE FF FF BB BB FF FF EE EE FF FF BB BB FF FF EE EE
FF FF BB BB FF FF EE EE > } image } if PT 4 eq { 16 16 1 [ 16 0 0 16 neg 0 16
] { < DF DF BF BF 7F 7F FE FE FD FD FB FB F7 F7 EF EF DF DF BF BF 7F 7F FE FE
FD FD FB FB F7 F7 EF EF > } image } if PT 5 eq { 16 16 1 [ 16 0 0 16 neg 0 16
] { < 7F 7F BF B F DF DF EF EF F7 F7 FB FB FD FD FE FE 7F 7F BF BF DF DF EF
EF F7 F7 FB FB FD FD FE FE > } image } if PT 6 eq { 16 16 1 [ 16 0 0 16 neg 0
16 ] { < BB BB BB BB BB BB BB BB BB BB BB BB BB BB BB BB BB BB BB BB BB BB BB
BB BB BB BB BB BB BB BB BB > } image } if PT 7 eq { 16 16 1 [ 16 0 0 16 neg 0
16 ] { < FF FF FF FF FF FF 00 00 FF FF FF FF FF FF 00 00 FF FF FF FF FF FF 00
00 FF FF FF FF FF FF 00 00 > } image } if PT 8 eq { 16 16 1 [ 16 0 0 16 neg 0
16 ] { < EE EE 47 47 83 83 C5 C5 EE EE 5C 5C 38 38 74 74 EE EE 47 47 83 83 C5
C5 EE EE 5C 5C 38 38 74 74 > } image } if PT 9 eq { 16 16 1 [ 16 0 0 16 neg 0
16 ] { < EF EF EF EF D7 D7 38 38 FE FE FE FE 7D 7D 83 83 EF EF EF EF D7 D7 38
38  FE FE FE FE 7D 7D 83 83 > } image } if PT 10 eq { 16 16 1 [ 16 0 0 16 neg
0 16 ] { <  EF EF EF EF EF EF 00 00 FE FE FE FE FE FE 00 00 EF EF EF EF EF EF
00 00 FE FE FE FE FE FE 00 00 > } image } if PT 11 eq { 16 16 1 [ 16 0 0 16
neg 0 16 ] { < F7 F7 B6 B6 D5 D5 E3 E3 D5 D5 B6 B6 F7 F7 FF FF 7F 7F 6B 6B 5D
5D 3E 3E 5D 5D 6B 6B 7F 7F FF FF > } image } if PT 12 eq { 16 16 1 [ 16 0 0
16 neg 0 16 ] { < E3 E3 DD DD BE BE BE BE BE BE DD DD E3 E3 FF FF 3E 3E DD DD
EB EB EB EB EB EB DD DD 3E 3E FF FF > } image } if PT 13 eq { 16 16 1 [ 16 0
0 16 neg 0 16 ] { <  FE FE 7D 7D BB BB D7 D7 EF EF D7 D7 BB BB 7D 7D FE FE 7D
7D BB BB D7 D7 EF EF D7 D7 BB BB 7D 7D > } image } if PT 14 eq { 16 16 1 [ 16
0 0 16 neg 0 16 ] { < 00 00 EE EF EE EF EE EF 0E E0 EE EE EE EE EE EE 00 EE
FE EE FE EE FE EE 00 00 FE EF FE EF FE EF > } image } if PT 15 eq { 16 16 1 [
16 0 0 16 neg 0 16 ] { < DD DD AA AA DD DD FF FF 77 77 AA AA 77 77 FF FF DD
DD AA AA DD DD FF FF 77 77 AA AA 77 77 FF FF > } image } if PT 16 eq { 16 16
1 [ 16 0 0 16 neg 0 16 ] { <  F1 F1 EE EE 1F 1F FF FF F1 F1 EE EE 1F 1F FF FF
F1 F1 EE EE 1F 1F FF FF F1 F1 EE EE 1F 1F FF FF > } image } if PT 17 eq { 16
16 1 [ 16 0 0 16 neg 0 16 ] { <  EE EE DD DD BB BB FF FF EE EE DD DD BB BB FF
 FF EE EE DD DD BB BB FF FF EE EE DD DD BB BB FF FF > } image } if PT 18 eq {
16 16 1 [ 16 0 0 16 neg 0 16 ] { <  BB BB DD DD EE EE FF FF BB BB DD DD EE EE
FF FF BB BB DD DD EE EE FF FF BB BB DD DD EE EE FF FF > } image } if PT 19 eq
{ 16 16 1 [ 16 0 0 16 neg 0 16 ] { < 1F FC 67 F3 7B EF BD DE BD DE DE BD E6
B3 F8 0F E6 B3 DE BD BD DE BD DE 7B EF 67 F3 1F FC 7F FF > } image } if PT
20 eq { 16 16 1 [ 16 0 0 16 neg 0 16 ] { < DD DD EE EE EE EE EE EE DD DD BB
BB BB BB BB BB DD DD EE EE EE EE EE EE DD DD BB BB BB BB BB BB > } image }
if PT 21 eq { 16 16 1 [ 16 0 0 16 neg 0 16 ] { < 0E 0E EF EF EF EF EF EF E0
E0 FE FE FE FE FE FE 0E 0E EF EF EF EF EF EF E0 E0 FE FE FE FE FE FE > }
image }  if PT 22 eq { 16 16 1 [ 16 0 0 16 neg 0 16 ] { < 70 70 F7 F7 F7 F7 F7
F7 07 07 7F 7F 7F 7F 7F 7F 70 70 F7 F7 F7 F7 F7 F7 07 07 7F 7F 7F 7F 7F 7F >
} image } if PT 23 eq  { 16 16 1 [ 16 0 0 16 neg 0 16 ] { < AA AA 55 55 A9 A9
D1 D1 E1 E1 D1 D1 A9 A9 55 55 AA AA 55 55 A9 A9 D1 D1 E1 E1 D1 D1 A9 A9 55 55
> } image } if PT 24 eq { 16 16 1 [ 16 0 0 16 neg 0 16 ] { < FF FE FF FC EA
A8 D5 54 EA A8 D5 54 E8 28 D4 54 E8 E8 D4 D4 E8 EA 54 D5 A8 EA 54 D5 00 C0 00
80 > } image } if PT 25 eq {  16 16 1 [ 16 0 0 16 neg 0 16 ] { < FF FE FF FC
FF F8 FF F0 F0 00 F0 00 F0 20 F0 60 F0 E0 F1 E0 F3 E0 F0 00 E0 00 C0 00 80 00
00 00 > } image } if gr } def /FA { /PT exch def gsave clip 0 0 translate 1 1
54 { 1 sub 47.2 mul /Xcurr exch def 1 1 74 { 1 sub 47.2 mul /Ycurr exch def
gsave Xcurr Ycurr translate PT DP gr } for } for gr newpath } def
/reencdict 24 dict def /ReEncode {reencdict begin /nco&na exch def
/nfnam exch def /basefontname exch def /basefontdict basefontname findfont def
/newfont basefontdict maxlength dict def basefontdict {exch dup /FID ne
{dup /Encoding eq {exch dup length array copy newfont 3 1 roll put} {exch
newfont 3 1 roll put} ifelse} {pop pop} ifelse } forall newfont
/FontName nfnam put nco&na aload pop nco&na length 2 idiv {newfont
/Encoding get 3 1 roll put} repeat nfnam newfont definefont pop end } def
/accvec [ 176 /agrave 181 /Agrave 190 /acircumflex 192 /Acircumflex
201 /adieresis 204 /Adieresis 209 /ccedilla 210 /Ccedilla 211 /eacute
212 /Eacute 213 /egrave 214 /Egrave 215 /ecircumflex 216 /Ecircumflex
217 /edieresis 218 /Edieresis 219 /icircumflex 220 /Icircumflex
221 /idieresis 222 /Idieresis 223 /ntilde 224 /Ntilde 226 /ocircumflex
228 /Ocircumflex 229 /odieresis 230 /Odieresis 231 /ucircumflex 236 /Ucircumflex
237 /udieresis 238 /Udieresis 239 /aring 242 /Aring 243 /ydieresis
244 /Ydieresis 246 /aacute 247 /Aacute 252 /ugrave 253 /Ugrave] def
/Times-Roman /Times-Roman accvec ReEncode
/Times-Italic /Times-Italic accvec ReEncode
/Times-Bold /Times-Bold accvec ReEncode
/Times-BoldItalic /Times-BoldItalic accvec ReEncode
/Helvetica /Helvetica accvec ReEncode
/Helvetica-Oblique /Helvetica-Oblique accvec ReEncode
/Helvetica-Bold /Helvetica-Bold accvec ReEncode
/Helvetica-BoldOblique /Helvetica-BoldOblique  accvec ReEncode
/Courier /Courier accvec ReEncode
/Courier-Oblique /Courier-Oblique accvec ReEncode
/Courier-Bold /Courier-Bold accvec ReEncode
/Courier-BoldOblique /Courier-BoldOblique accvec ReEncode
/oshow {gsave [] 0 sd true charpath stroke gr} def
/stwn { /fs exch def /fn exch def /text exch def fn findfont fs sf
 text sw pop xs add /xs exch def} def
/stwb { /fs exch def /fn exch def /nbas exch def /textf exch def
textf length /tlen exch def nbas tlen gt {/nbas tlen def} if
fn findfont fs sf textf dup length nbas sub nbas getinterval sw
pop neg xs add /xs exch def} def
/accspe [ 65 /plusminus 66 /bar 67 /existential 68 /universal
69 /exclam 70 /numbersign 71 /greater 72 /question 73 /integral
74 /colon 75 /semicolon 76 /less 77 /bracketleft 78 /bracketright
79 /greaterequal 80 /braceleft 81 /braceright 82 /radical
83 /spade 84 /heart 85 /diamond 86 /club 87 /lessequal
88 /multiply 89 /percent 90 /infinity 48 /circlemultiply 49 /circleplus
50 /emptyset 51 /lozenge 52 /bullet 53 /arrowright 54 /arrowup
55 /arrowleft 56 /arrowdown 57 /arrowboth 48 /degree 44 /comma 43 /plus
 45 /angle 42 /angleleft 47 /divide 61 /notequal 40 /equivalence 41 /second
 97 /approxequal 98 /congruent 99 /perpendicular 100 /partialdiff 101 /florin
 102 /intersection 103 /union 104 /propersuperset 105 /reflexsuperset
 106 /notsubset 107 /propersubset 108 /reflexsubset 109 /element 110 /notelement
 111 /gradient 112 /logicaland 113 /logicalor 114 /arrowdblboth
 115 /arrowdblleft 116 /arrowdblup 117 /arrowdblright 118 /arrowdbldown
 119 /ampersand 120 /omega1 121 /similar 122 /aleph ] def
/Symbol /Special accspe ReEncode
 gsave  .25 .25 scale  gsave 0 0 t black [] 0 sd 1 lw 4 lw 1270 493 363 1287 bl
 1735 2120 0 0 C 1270 493 363 1287 C NC 1 lw 363 1287 m 493 Y s 3 lw 397 1332 m
 -34 X s 380 1376 m -17 X s 380 1421 m -17 X s 380 1466 m -17 X s 397 1511 m -34
 X s 380 1556 m -17 X s 380 1601 m -17 X s 380 1645 m -17 X s 397 1690 m -34 X s
 397 1332 m -34 X s 397 1690 m -34 X s 380 1735 m -17 X s
 /xs 0 def 
(-0.4)
 /Helvetica     62 stwn 
 gsave  338 1309
 t   0 r  xs neg 0 t 0 0 m
 /Helvetica findfont   62 sf 0    0 m 
(-0.4)
 show 
 gr 
 /xs 0 def 
(-0.2)
 /Helvetica     62 stwn 
 gsave  338 1488
 t   0 r  xs neg 0 t 0 0 m
 /Helvetica findfont   62 sf 0    0 m 
(-0.2)
 show 
 gr 
 /xs 0 def 
(0)
 /Helvetica     62 stwn 
 gsave  338 1668
 t   0 r  xs neg 0 t 0 0 m
 /Helvetica findfont   62 sf 0    0 m 
(0)
 show 
 gr  1 lw 363 1287 m 1270 X s 3 lw 554 1304 m -17 Y s 666 1304 m -17 Y s 745
 1304 m -17 Y s 807 1304 m -17 Y s 857 1304 m -17 Y s 899 1304 m -17 Y s 936
 1304 m -17 Y s 969 1304 m -17 Y s 998 1321 m -34 Y s
 /xs 0 def 
(10)
 /Helvetica     62 stwn 
 gsave  998 1189
 t   0 r  xs 2 div neg 0 t 0 0 m
 /Helvetica findfont   62 sf 0    0 m 
(10)
 show 
 gr 
 /xs 0 def 
(2)
 /Helvetica     50 stwn 
 gsave  1054 1235
 t   0 r  xs 2 div neg 0 t 0 0 m
 /Helvetica findfont   50 sf 0    0 m 
(2)
 show 
 gr  1189 1304 m -17 Y s 1301 1304 m -17 Y s 1380 1304 m -17 Y s 1441 1304 m -17
 Y s 1492 1304 m -17 Y s 1534 1304 m -17 Y s 1571 1304 m -17 Y s 1603 1304 m -17
 Y s 1633 1321 m -34 Y s
 /xs 0 def 
(10)
 /Helvetica     62 stwn 
 gsave  1633 1189
 t   0 r  xs 2 div neg 0 t 0 0 m
 /Helvetica findfont   62 sf 0    0 m 
(10)
 show 
 gr 
 /xs 0 def 
(3)
 /Helvetica     50 stwn 
 gsave  1689 1235
 t   0 r  xs 2 div neg 0 t 0 0 m
 /Helvetica findfont   50 sf 0    0 m 
(3)
 show 
 gr  1270 493 363 1287 C 2 lw 457 1327 m 37 Y s 457 1390 m 36 Y s /w 26
 def /w2 {w 2 div} def /w3 {w 3 div} def 457 1377 m20 646 1362 m 33 Y s 646 1421
 m 33 Y s 646 1408 m20 835 1400 m 8 Y s 835 1434 m 8 Y s 835 1421 m20 1024 1458
 m20 1216 1490 m 18 Y s 1216 1534 m 19 Y s 1216 1521 m20 1407 1593 m 22 Y s 1407
 1641 m 23 Y s 1407 1628 m20 1604 1328 m 140 Y s 1604 1494 m 140 Y s 1604 1481
 m20 4 lw 457 1377 m20 646 1408 m20 835 1421 m20 1024 1458 m20 1216 1506 m 2 Y s
 1216 1534 m 3 Y s 1203 1506 m 26 X s 1203 1537 m 26 X s 1216 1521 m20 1407 1611
 m 4 Y s 1407 1641 m 5 Y s 1394 1611 m 26 X s 1394 1646 m 26 X s 1407 1628 m20
 1604 1329 m 139 Y s 1604 1494 m 140 Y s 1591 1329 m 27 X s 1591 1634 m 27 X s
 1604 1481 m20 457 1390 m 189 25 d 189 10 d 189 35 d 192 71 d 191 94 d 197 -18 d
 s /w 4 def /w2 {w 2 div} def /w3 {w 3 div} def 457 1390 646 1415 835 1425 1024
 1460 1216 1531 1407 1625 1604 1607 7 { m20} R [12 12] 0 sd 457 1488 m 189 -12 d
 189 11 d 189 20 d 192 70 d 191 24 d 197 57 d s [] 0 sd 457 1488 646 1476 835
 1487 1024 1507 1216 1577 1407 1601 1604 1658 7 { m20} R [4 8] 0 sd 457 1500 m
 189 19 d 189 43 d 189 38 d 192 101 d 191 14 d 197 16 d s [] 0 sd 457 1500 646
 1519 835 1562 1024 1600 1216 1701 1407 1715 1604 1731 7 { m20} R 1735 2120 0 0
 C 1270 493 363 1287 C 1735 2120 0 0 C /w 32
 def /w2 {w 2 div} def /w3 {w 3 div} def 389 1932 m20 1270 493 363 1287 C 580
 1932 m 57 X s [12 12] 0 sd 962 1932 m 62 X s [4 8] 0 sd 1282 1932 m 45 X s 1735
 2120 0 0 C 1270 493 363 1287 C 1735 2120 0 0 C 1270 493 363 1287 C 1735 2120 0
 0 C [] 0 sd 615 1928 m 68 X s 1270 493 363 1287 C 1735 2120 0 0 C 1270 493 363
 1287 C 1735 2120 0 0 C 1270 493 363 1287 C 1735 2120 0 0 C [12 12] 0 sd 998
 1928 m 80 X s 1270 493 363 1287 C 1735 2120 0 0 C 1270 493 363 1287 C 1735 2120
 0 0 C 1270 493 363 1287 C 1735 2120 0 0 C [4 8] 0 sd 1324 1928 m 63 X s 1270
 493 363 1287 C 1735 2120 0 0 C 1270 493 363 1287 C 1735 2120 0 0 C
 gsave  427 1915
 t   0 r 0 0 m
 /Times-Bold findfont   42 sf 0    0 m 
(ZEUS 95)
 show 
 gr  1270 493 363 1287 C 1735 2120 0 0 C 1270 493 363 1287 C 1735 2120 0 0 C
 gsave  708 1915
 t   0 r 0 0 m
 /Times-Bold findfont   42 sf 0    0 m 
(ARIADNE 4.8)
 show 
 gr  1270 493 363 1287 C 1735 2120 0 0 C 1270 493 363 1287 C 1735 2120 0 0 C
 gsave  1090 1915
 t   0 r 0 0 m
 /Times-Bold findfont   42 sf 0    0 m 
(LEPTO 6.5)
 show 
 gr  1270 493 363 1287 C 1735 2120 0 0 C 1270 493 363 1287 C 1735 2120 0 0 C
 gsave  1400 1915
 t   0 r 0 0 m
 /Times-Bold findfont   42 sf 0    0 m 
(HERWIG 5.9)
 show 
 gr  1270 493 363 1287 C 1735 2120 0 0 C 1270 493 363 1287 C 1735 2120 0 0 C
 gsave  110 1807
 t   0 r 0 0 m
 /Helvetica findfont   62 sf 0    0 m 
(\074 x \076 :)
 show 
 gr  1270 493 363 1287 C 1735 2120 0 0 C 1270 493 363 1287 C 1735 2120 0 0 C
 gsave  389 1807
 t   0 r 0 0 m
 /Helvetica findfont   47 sf 0    0 m 
(0.0012)
 show 
 gr  1270 493 363 1287 C 1735 2120 0 0 C 1270 493 363 1287 C 1735 2120 0 0 C
 gsave  580 1807
 t   0 r 0 0 m
 /Helvetica findfont   47 sf 0    0 m 
(0.003)
 show 
 gr  1270 493 363 1287 C 1735 2120 0 0 C 1270 493 363 1287 C 1735 2120 0 0 C
 gsave  777 1807
 t   0 r 0 0 m
 /Helvetica findfont   47 sf 0    0 m 
(0.004)
 show 
 gr  1270 493 363 1287 C 1735 2120 0 0 C 1270 493 363 1287 C 1735 2120 0 0 C
 gsave  984 1807
 t   0 r 0 0 m
 /Helvetica findfont   47 sf 0    0 m 
(0.005)
 show 
 gr  1270 493 363 1287 C 1735 2120 0 0 C 1270 493 363 1287 C 1735 2120 0 0 C
 gsave  1160 1807
 t   0 r 0 0 m
 /Helvetica findfont   47 sf 0    0 m 
(0.016)
 show 
 gr  1270 493 363 1287 C 1735 2120 0 0 C 1270 493 363 1287 C 1735 2120 0 0 C
 gsave  1358 1807
 t   0 r 0 0 m
 /Helvetica findfont   47 sf 0    0 m 
(0.024)
 show 
 gr  1270 493 363 1287 C 1735 2120 0 0 C 1270 493 363 1287 C 1735 2120 0 0 C
 gsave  1534 1807
 t   0 r 0 0 m
 /Helvetica findfont   47 sf 0    0 m 
(0.025)
 show 
 gr  1270 493 363 1287 C 1735 2120 0 0 C 1270 493 363 1287 C 1735 2120 0 0 C
 gsave  435 1690
 t   0 r 0 0 m
 /Helvetica findfont   70 sf 0    0 m 
(\(a\))
 show 
 gr  1270 493 363 1287 C 1735 2120 0 0 C
 /xs 0 def 
(\074 Q)
 /Helvetica     78 stwn 
(2)
 /Helvetica     55 stwn 
( \076, GeV\040)
 /Helvetica     78 stwn 
(2)
 /Helvetica     55 stwn 
 gsave  1633 1085
 t   0 r  xs neg 0 t 0 0 m
 /Helvetica findfont   78 sf 0    0 m 
(\074 Q)
 show 
 currentpoint pop 0 t 
 /Helvetica findfont   55 sf 0   39 m 
(2)
 show 
 currentpoint pop 0 t 
 /Helvetica findfont   78 sf 0    0 m 
( \076, GeV\040)
 show 
 currentpoint pop 0 t 
 /Helvetica findfont   55 sf 0   39 m 
(2)
 show 
 gr  1270 493 363 1287 C 1735 2120 0 0 C 1270 493 363 1287 C 1735 2120 0 0 C
 gsave  57 1529
 t   0 r 0 0 m
 /Symbol findfont   93 sf 0    0 m 
(k)
 show 
 gr  1270 493 363 1287 C NC [] 0 sd 1270 494 363 453 bl 1735 2120 0 0 C 1270 494
 363 453 C NC 1 lw 363 453 m 494 Y s 3 lw 397 498 m -34 X s 380 543 m -17 X s
 380 588 m -17 X s 380 633 m -17 X s 397 678 m -34 X s 380 723 m -17 X s 380 767
 m -17 X s 380 812 m -17 X s 397 857 m -34 X s 397 498 m -34 X s 397 857 m -34 X
 s 380 902 m -17 X s
 /xs 0 def 
(-0.4)
 /Helvetica     62 stwn 
 gsave  338 476
 t   0 r  xs neg 0 t 0 0 m
 /Helvetica findfont   62 sf 0    0 m 
(-0.4)
 show 
 gr 
 /xs 0 def 
(-0.2)
 /Helvetica     62 stwn 
 gsave  338 655
 t   0 r  xs neg 0 t 0 0 m
 /Helvetica findfont   62 sf 0    0 m 
(-0.2)
 show 
 gr 
 /xs 0 def 
(0)
 /Helvetica     62 stwn 
 gsave  338 834
 t   0 r  xs neg 0 t 0 0 m
 /Helvetica findfont   62 sf 0    0 m 
(0)
 show 
 gr  1 lw 363 453 m 1270 X s 3 lw 363 470 m -17 Y s 440 470 m -17 Y s 505 470 m
 -17 Y s 562 470 m -17 Y s 612 470 m -17 Y s 657 487 m -34 Y s
 /xs 0 def 
(10)
 /Helvetica     62 stwn 
 gsave  634 356
 t   0 r  xs 2 div neg 0 t 0 0 m
 /Helvetica findfont   62 sf 0    0 m 
(10)
 show 
 gr 
 /xs 0 def 
(-3)
 /Helvetica     50 stwn 
 gsave  708 401
 t   0 r  xs 2 div neg 0 t 0 0 m
 /Helvetica findfont   50 sf 0    0 m 
(-3)
 show 
 gr  950 470 m -17 Y s 1122 470 m -17 Y s 1244 470 m -17 Y s 1339 470 m -17 Y s
 1416 470 m -17 Y s 1481 470 m -17 Y s 1538 470 m -17 Y s 1588 470 m -17 Y s
 1633 487 m -34 Y s
 /xs 0 def 
(10)
 /Helvetica     62 stwn 
 gsave  1610 356
 t   0 r  xs 2 div neg 0 t 0 0 m
 /Helvetica findfont   62 sf 0    0 m 
(10)
 show 
 gr 
 /xs 0 def 
(-2)
 /Helvetica     50 stwn 
 gsave  1684 401
 t   0 r  xs 2 div neg 0 t 0 0 m
 /Helvetica findfont   50 sf 0    0 m 
(-2)
 show 
 gr  1270 494 363 453 C 2 lw 597 555 m 19 Y s 597 600 m 20 Y s /w 26
 def /w2 {w 2 div} def /w3 {w 3 div} def 597 587 m20 888 608 m 21 Y s 888 656 m
 21 Y s 888 642 m20 1360 653 m 40 Y s 1360 719 m 40 Y s 1360 706 m20 4 lw 597
 587 m20 888 642 m20 1360 706 m20 597 600 m 291 46 d 472 69 d s /w 4
 def /w2 {w 2 div} def /w3 {w 3 div} def 597 600 888 646 1360 715 3 { m20} R
 [12 12] 0 sd 597 694 m 291 42 d 472 67 d s [] 0 sd 597 694 888 736 1360 803 3 {
 m20} R [4 8] 0 sd 597 716 m 291 32 d 472 36 d s [] 0 sd 597 716 888 748 1360
 784 3 { m20} R 1735 2120 0 0 C
 /xs 0 def 
(\074 x \076)
 /Helvetica     78 stwn 
 gsave  1633 274
 t   0 r  xs neg 0 t 0 0 m
 /Helvetica findfont   78 sf 0    0 m 
(\074 x \076)
 show 
 gr  1270 494 363 453 C 1735 2120 0 0 C 1270 494 363 453 C 1735 2120 0 0 C
 gsave  66 696
 t   0 r 0 0 m
 /Symbol findfont   93 sf 0    0 m 
(k)
 show 
 gr  1270 494 363 453 C 1735 2120 0 0 C 1270 494 363 453 C 1735 2120 0 0 C
 gsave  69 974
 t   0 r 0 0 m
 /Helvetica findfont   62 sf 0    0 m 
(\074 Q)
 show 
 currentpoint pop 0 t 
 /Helvetica findfont   43 sf 0   31 m 
(2)
 show 
 currentpoint pop 0 t 
 /Helvetica findfont   62 sf 0    0 m 
( \076 :)
 show 
 gr  1270 494 363 453 C 1735 2120 0 0 C 1270 494 363 453 C 1735 2120 0 0 C
 gsave  578 974
 t   0 r 0 0 m
 /Helvetica findfont   47 sf 0    0 m 
(21)
 show 
 gr  1270 494 363 453 C 1735 2120 0 0 C 1270 494 363 453 C 1735 2120 0 0 C
 gsave  881 974
 t   0 r 0 0 m
 /Helvetica findfont   47 sf 0    0 m 
(27)
 show 
 gr  1270 494 363 453 C 1735 2120 0 0 C 1270 494 363 453 C 1735 2120 0 0 C
 gsave  1339 974
 t   0 r 0 0 m
 /Helvetica findfont   47 sf 0    0 m 
(38)
 show 
 gr  1270 494 363 453 C 1735 2120 0 0 C 1270 494 363 453 C 1735 2120 0 0 C
 gsave  440 857
 t   0 r 0 0 m
 /Helvetica findfont   70 sf 0    0 m 
(\(b\))
 show 
 gr  1270 494 363 453 C
 gr  gr 
showpage
end
%%EndDocument


==> brook.7 <==
%%BeginDocument: eps/cplotnbw.eps
80 dict begin
/s {stroke} def /l {lineto} def /m {moveto} def /t {translate} def
/sw {stringwidth} def /r {rotate} def /rl {roll}  def /R {repeat} def
/d {rlineto} def /rm {rmoveto} def /gr {grestore} def /f {eofill} def
/c {setrgbcolor} def /lw {setlinewidth} def /sd {setdash} def
/cl {closepath} def /sf {scalefont setfont} def /black {0 setgray} def
/box {m dup 0 exch d exch 0 d 0 exch neg d cl} def
/NC{systemdict begin initclip end}def/C{NC box clip newpath}def
/bl {box s} def /bf {box f} def /Y { 0 exch d} def /X { 0 d} def 
/mp {newpath /y exch def /x exch def} def
/side {[w .77 mul w .23 mul] .385 w mul sd w 0 l currentpoint t -144 r} def
/mr {mp x y w2 0 360 arc} def /m24 {mr s} def /m20 {mr f} def
/mb {mp x y w2 add m w2 neg 0 d 0 w neg d w 0 d 0 w d cl} def
/mt {mp x y w2 add m w2 neg w neg d w 0 d cl} def
/m21 {mb f} def /m25 {mb s} def /m22 {mt f} def /m26 {mt s} def
/m23 {mp x y w2 sub m w2 w d w neg 0 d cl f} def
/m27 {mp x y w2 add m w3 neg w2 neg d w3 w2 neg d w3  w2 d cl s} def
/m28 {mp x w2 sub y w2 sub w3 add m w3 0 d 0 w3 neg d w3 0 d 0 w3 d w3 0 d
 0 w3 d w3 neg 0 d 0 w3 d w3 neg 0 d
 0 w3 neg d w3 neg 0 d cl s } def
/m29 {mp gsave x w2 sub y w2 add w3 sub m currentpoint t
 4 {side} repeat cl fill gr} def
/m30 {mp gsave x w2 sub y w2 add w3 sub m currentpoint t
 5 {side} repeat s gr} def
/m31 {mp x y w2 sub m 0 w d x w2 sub y m w 0 d
 x w2 sub y w2 add m w w neg d x w2 sub y w2
 sub m w w d s} def
/m2 {mp x y w2 sub m 0 w d x w2 sub y m w 0 d s} def
/m5 {mp x w2 sub y w2 sub m w w d x w2 sub y w2 add m w w neg d s} def
/DP {/PT exch def gsave 47.2 47.2 scale PT 1  eq { 16 16 1 [ 16 0 0 16 neg 0 16
] { < AA AA 55 55 AA AA 55 55 AA AA 55 55 AA AA 55 55 AA AA 55 55 AA AA 55 55
AA AA 55 55 AA AA 55 55 > } image } if PT 2 eq { 16 16 1 [ 16 0 0 16 neg 0 16
] { < BB BB EE EE BB BB EE EE BB BB EE EE BB BB EE EE BB BB EE EE BB BB EE EE
BB BB EE EE BB BB EE EE > } image } if PT 3 eq { 16 16 1 [ 16 0 0 16 neg 0 16
] { < FF FF BB BB FF FF EE EE FF FF BB BB FF FF EE EE FF FF BB BB FF FF EE EE
FF FF BB BB FF FF EE EE > } image } if PT 4 eq { 16 16 1 [ 16 0 0 16 neg 0 16
] { < DF DF BF BF 7F 7F FE FE FD FD FB FB F7 F7 EF EF DF DF BF BF 7F 7F FE FE
FD FD FB FB F7 F7 EF EF > } image } if PT 5 eq { 16 16 1 [ 16 0 0 16 neg 0 16
] { < 7F 7F BF B F DF DF EF EF F7 F7 FB FB FD FD FE FE 7F 7F BF BF DF DF EF
EF F7 F7 FB FB FD FD FE FE > } image } if PT 6 eq { 16 16 1 [ 16 0 0 16 neg 0
16 ] { < BB BB BB BB BB BB BB BB BB BB BB BB BB BB BB BB BB BB BB BB BB BB BB
BB BB BB BB BB BB BB BB BB > } image } if PT 7 eq { 16 16 1 [ 16 0 0 16 neg 0
16 ] { < FF FF FF FF FF FF 00 00 FF FF FF FF FF FF 00 00 FF FF FF FF FF FF 00
00 FF FF FF FF FF FF 00 00 > } image } if PT 8 eq { 16 16 1 [ 16 0 0 16 neg 0
16 ] { < EE EE 47 47 83 83 C5 C5 EE EE 5C 5C 38 38 74 74 EE EE 47 47 83 83 C5
C5 EE EE 5C 5C 38 38 74 74 > } image } if PT 9 eq { 16 16 1 [ 16 0 0 16 neg 0
16 ] { < EF EF EF EF D7 D7 38 38 FE FE FE FE 7D 7D 83 83 EF EF EF EF D7 D7 38
38  FE FE FE FE 7D 7D 83 83 > } image } if PT 10 eq { 16 16 1 [ 16 0 0 16 neg
0 16 ] { <  EF EF EF EF EF EF 00 00 FE FE FE FE FE FE 00 00 EF EF EF EF EF EF
00 00 FE FE FE FE FE FE 00 00 > } image } if PT 11 eq { 16 16 1 [ 16 0 0 16
neg 0 16 ] { < F7 F7 B6 B6 D5 D5 E3 E3 D5 D5 B6 B6 F7 F7 FF FF 7F 7F 6B 6B 5D
5D 3E 3E 5D 5D 6B 6B 7F 7F FF FF > } image } if PT 12 eq { 16 16 1 [ 16 0 0
16 neg 0 16 ] { < E3 E3 DD DD BE BE BE BE BE BE DD DD E3 E3 FF FF 3E 3E DD DD
EB EB EB EB EB EB DD DD 3E 3E FF FF > } image } if PT 13 eq { 16 16 1 [ 16 0
0 16 neg 0 16 ] { <  FE FE 7D 7D BB BB D7 D7 EF EF D7 D7 BB BB 7D 7D FE FE 7D
7D BB BB D7 D7 EF EF D7 D7 BB BB 7D 7D > } image } if PT 14 eq { 16 16 1 [ 16
0 0 16 neg 0 16 ] { < 00 00 EE EF EE EF EE EF 0E E0 EE EE EE EE EE EE 00 EE
FE EE FE EE FE EE 00 00 FE EF FE EF FE EF > } image } if PT 15 eq { 16 16 1 [
16 0 0 16 neg 0 16 ] { < DD DD AA AA DD DD FF FF 77 77 AA AA 77 77 FF FF DD
DD AA AA DD DD FF FF 77 77 AA AA 77 77 FF FF > } image } if PT 16 eq { 16 16
1 [ 16 0 0 16 neg 0 16 ] { <  F1 F1 EE EE 1F 1F FF FF F1 F1 EE EE 1F 1F FF FF
F1 F1 EE EE 1F 1F FF FF F1 F1 EE EE 1F 1F FF FF > } image } if PT 17 eq { 16
16 1 [ 16 0 0 16 neg 0 16 ] { <  EE EE DD DD BB BB FF FF EE EE DD DD BB BB FF
 FF EE EE DD DD BB BB FF FF EE EE DD DD BB BB FF FF > } image } if PT 18 eq {
16 16 1 [ 16 0 0 16 neg 0 16 ] { <  BB BB DD DD EE EE FF FF BB BB DD DD EE EE
FF FF BB BB DD DD EE EE FF FF BB BB DD DD EE EE FF FF > } image } if PT 19 eq
{ 16 16 1 [ 16 0 0 16 neg 0 16 ] { < 1F FC 67 F3 7B EF BD DE BD DE DE BD E6
B3 F8 0F E6 B3 DE BD BD DE BD DE 7B EF 67 F3 1F FC 7F FF > } image } if PT
20 eq { 16 16 1 [ 16 0 0 16 neg 0 16 ] { < DD DD EE EE EE EE EE EE DD DD BB
BB BB BB BB BB DD DD EE EE EE EE EE EE DD DD BB BB BB BB BB BB > } image }
if PT 21 eq { 16 16 1 [ 16 0 0 16 neg 0 16 ] { < 0E 0E EF EF EF EF EF EF E0
E0 FE FE FE FE FE FE 0E 0E EF EF EF EF EF EF E0 E0 FE FE FE FE FE FE > }
image }  if PT 22 eq { 16 16 1 [ 16 0 0 16 neg 0 16 ] { < 70 70 F7 F7 F7 F7 F7
F7 07 07 7F 7F 7F 7F 7F 7F 70 70 F7 F7 F7 F7 F7 F7 07 07 7F 7F 7F 7F 7F 7F >
} image } if PT 23 eq  { 16 16 1 [ 16 0 0 16 neg 0 16 ] { < AA AA 55 55 A9 A9
D1 D1 E1 E1 D1 D1 A9 A9 55 55 AA AA 55 55 A9 A9 D1 D1 E1 E1 D1 D1 A9 A9 55 55
> } image } if PT 24 eq { 16 16 1 [ 16 0 0 16 neg 0 16 ] { < FF FE FF FC EA
A8 D5 54 EA A8 D5 54 E8 28 D4 54 E8 E8 D4 D4 E8 EA 54 D5 A8 EA 54 D5 00 C0 00
80 > } image } if PT 25 eq {  16 16 1 [ 16 0 0 16 neg 0 16 ] { < FF FE FF FC
FF F8 FF F0 F0 00 F0 00 F0 20 F0 60 F0 E0 F1 E0 F3 E0 F0 00 E0 00 C0 00 80 00
00 00 > } image } if gr } def /FA { /PT exch def gsave clip 0 0 translate 1 1
54 { 1 sub 47.2 mul /Xcurr exch def 1 1 74 { 1 sub 47.2 mul /Ycurr exch def
gsave Xcurr Ycurr translate PT DP gr } for } for gr newpath } def
/reencdict 24 dict def /ReEncode {reencdict begin /nco&na exch def
/nfnam exch def /basefontname exch def /basefontdict basefontname findfont def
/newfont basefontdict maxlength dict def basefontdict {exch dup /FID ne
{dup /Encoding eq {exch dup length array copy newfont 3 1 roll put} {exch
newfont 3 1 roll put} ifelse} {pop pop} ifelse } forall newfont
/FontName nfnam put nco&na aload pop nco&na length 2 idiv {newfont
/Encoding get 3 1 roll put} repeat nfnam newfont definefont pop end } def
/accvec [ 176 /agrave 181 /Agrave 190 /acircumflex 192 /Acircumflex
201 /adieresis 204 /Adieresis 209 /ccedilla 210 /Ccedilla 211 /eacute
212 /Eacute 213 /egrave 214 /Egrave 215 /ecircumflex 216 /Ecircumflex
217 /edieresis 218 /Edieresis 219 /icircumflex 220 /Icircumflex
221 /idieresis 222 /Idieresis 223 /ntilde 224 /Ntilde 226 /ocircumflex
228 /Ocircumflex 229 /odieresis 230 /Odieresis 231 /ucircumflex 236 /Ucircumflex
237 /udieresis 238 /Udieresis 239 /aring 242 /Aring 243 /ydieresis
244 /Ydieresis 246 /aacute 247 /Aacute 252 /ugrave 253 /Ugrave] def
/Times-Roman /Times-Roman accvec ReEncode
/Times-Italic /Times-Italic accvec ReEncode
/Times-Bold /Times-Bold accvec ReEncode
/Times-BoldItalic /Times-BoldItalic accvec ReEncode
/Helvetica /Helvetica accvec ReEncode
/Helvetica-Oblique /Helvetica-Oblique accvec ReEncode
/Helvetica-Bold /Helvetica-Bold accvec ReEncode
/Helvetica-BoldOblique /Helvetica-BoldOblique  accvec ReEncode
/Courier /Courier accvec ReEncode
/Courier-Oblique /Courier-Oblique accvec ReEncode
/Courier-Bold /Courier-Bold accvec ReEncode
/Courier-BoldOblique /Courier-BoldOblique accvec ReEncode
/oshow {gsave [] 0 sd true charpath stroke gr} def
/stwn { /fs exch def /fn exch def /text exch def fn findfont fs sf
 text sw pop xs add /xs exch def} def
/stwb { /fs exch def /fn exch def /nbas exch def /textf exch def
textf length /tlen exch def nbas tlen gt {/nbas tlen def} if
fn findfont fs sf textf dup length nbas sub nbas getinterval sw
pop neg xs add /xs exch def} def
/accspe [ 65 /plusminus 66 /bar 67 /existential 68 /universal
69 /exclam 70 /numbersign 71 /greater 72 /question 73 /integral
74 /colon 75 /semicolon 76 /less 77 /bracketleft 78 /bracketright
79 /greaterequal 80 /braceleft 81 /braceright 82 /radical
83 /spade 84 /heart 85 /diamond 86 /club 87 /lessequal
88 /multiply 89 /percent 90 /infinity 48 /circlemultiply 49 /circleplus
50 /emptyset 51 /lozenge 52 /bullet 53 /arrowright 54 /arrowup
55 /arrowleft 56 /arrowdown 57 /arrowboth 48 /degree 44 /comma 43 /plus
 45 /angle 42 /angleleft 47 /divide 61 /notequal 40 /equivalence 41 /second
 97 /approxequal 98 /congruent 99 /perpendicular 100 /partialdiff 101 /florin
 102 /intersection 103 /union 104 /propersuperset 105 /reflexsuperset
 106 /notsubset 107 /propersubset 108 /reflexsubset 109 /element 110 /notelement
 111 /gradient 112 /logicaland 113 /logicalor 114 /arrowdblboth
 115 /arrowdblleft 116 /arrowdblup 117 /arrowdblright 118 /arrowdbldown
 119 /ampersand 120 /omega1 121 /similar 122 /aleph ] def
/Symbol /Special accspe ReEncode
 gsave  .25 .25 scale  gsave 0 0 t black [] 0 sd 1 lw 2 lw 595 850 210 136 bl
 595 850 210 136 C NC 1 lw 210 136 m 850 Y s 2 lw 232 278 m -22 X s 221 334 m
 -11 X s 221 391 m -11 X s 221 448 m -11 X s 221 504 m -11 X s 232 561 m -22 X s
 221 618 m -11 X s 221 674 m -11 X s 221 731 m -11 X s 221 788 m -11 X s 232 844
 m -22 X s 232 278 m -22 X s 221 221 m -11 X s 221 164 m -11 X s 232 844 m -22 X
 s 221 901 m -11 X s 221 958 m -11 X s
 /xs 0 def 
(0.4)
 /Helvetica-Bold     37 stwn 
 gsave  176 264
 t   0 r  xs neg 0 t 0 0 m
 /Helvetica-Bold findfont   37 sf 0    0 m 
(0.4)
 show 
 gr 
 /xs 0 def 
(0.5)
 /Helvetica-Bold     37 stwn 
 gsave  176 547
 t   0 r  xs neg 0 t 0 0 m
 /Helvetica-Bold findfont   37 sf 0    0 m 
(0.5)
 show 
 gr 
 /xs 0 def 
(0.6)
 /Helvetica-Bold     37 stwn 
 gsave  176 831
 t   0 r  xs neg 0 t 0 0 m
 /Helvetica-Bold findfont   37 sf 0    0 m 
(0.6)
 show 
 gr  1 lw 210 136 m 595 X s 2 lw 210 159 m -23 Y s 239 147 m -11 Y s 269 147 m
 -11 Y s 299 147 m -11 Y s 329 147 m -11 Y s 358 159 m -23 Y s 388 147 m -11 Y s
 418 147 m -11 Y s 448 147 m -11 Y s 477 147 m -11 Y s 507 159 m -23 Y s 537 147
 m -11 Y s 567 147 m -11 Y s 596 147 m -11 Y s 626 147 m -11 Y s 656 159 m -23 Y
 s 686 147 m -11 Y s 715 147 m -11 Y s 745 147 m -11 Y s 775 147 m -11 Y s 805
 159 m -23 Y s 210 159 m -23 Y s 805 159 m -23 Y s
 /xs 0 def 
(0.1)
 /Helvetica-Bold     37 stwn 
 gsave  210 86
 t   0 r  xs 2 div neg 0 t 0 0 m
 /Helvetica-Bold findfont   37 sf 0    0 m 
(0.1)
 show 
 gr 
 /xs 0 def 
(0.11)
 /Helvetica-Bold     37 stwn 
 gsave  358 86
 t   0 r  xs 2 div neg 0 t 0 0 m
 /Helvetica-Bold findfont   37 sf 0    0 m 
(0.11)
 show 
 gr 
 /xs 0 def 
(0.12)
 /Helvetica-Bold     37 stwn 
 gsave  507 86
 t   0 r  xs 2 div neg 0 t 0 0 m
 /Helvetica-Bold findfont   37 sf 0    0 m 
(0.12)
 show 
 gr 
 /xs 0 def 
(0.13)
 /Helvetica-Bold     37 stwn 
 gsave  656 86
 t   0 r  xs 2 div neg 0 t 0 0 m
 /Helvetica-Bold findfont   37 sf 0    0 m 
(0.13)
 show 
 gr 
 /xs 0 def 
(0.14)
 /Helvetica-Bold     37 stwn 
 gsave  805 86
 t   0 r  xs 2 div neg 0 t 0 0 m
 /Helvetica-Bold findfont   37 sf 0    0 m 
(0.14)
 show 
 gr  595 850 210 136 C 850 1020 0 0 C
 /xs 0 def 
(a)
 /Symbol     43 stwn 
(s)
 /Helvetica-Bold     30 stwn 
(\(M)
 /Helvetica-Bold     43 stwn 
(Z)
 /Helvetica-Bold     30 stwn 
(\))
 /Helvetica-Bold     43 stwn 
 gsave  805 25
 t   0 r  xs neg 0 t 0 0 m
 /Symbol findfont   43 sf 0    0 m 
(a)
 show 
 currentpoint pop 0 t 
 /Helvetica-Bold findfont   30 sf 0  -14 m 
(s)
 show 
 currentpoint pop 0 t 
 /Helvetica-Bold findfont   43 sf 0    0 m 
(\(M)
 show 
 currentpoint pop 0 t 
 /Helvetica-Bold findfont   30 sf 0  -14 m 
(Z)
 show 
 currentpoint pop 0 t 
 /Helvetica-Bold findfont   43 sf 0    0 m 
(\))
 show 
 gr 
 /xs 0 def 
(a)
 /Symbol     43 stwn 
(0)
 /Helvetica-Bold     30 stwn 
(\()
 /Helvetica-Bold     43 stwn 
(m)
 /Symbol     43 stwn 
(I)
 /Symbol     30 stwn 
( = 2 GeV\))
 /Helvetica-Bold     43 stwn 
 gsave  51 986
 t  90 r  xs neg 0 t 0 0 m
 /Symbol findfont   43 sf 0    0 m 
(a)
 show 
 currentpoint pop 0 t 
/Symbol findfont   43 sf 
(a)
 dup length 1 sub 1 getinterval 
 stringwidth pop 2 div neg    0 rm 
 /Helvetica-Bold findfont   30 sf 0   30 rm 
(_)
 stringwidth pop 2 div neg 0 rm 
(_)
 show
 /Helvetica-Bold findfont   30 sf 0  -14 m 
(0)
 show 
 currentpoint pop 0 t 
 /Helvetica-Bold findfont   43 sf 0    0 m 
(\()
 show 
 currentpoint pop 0 t 
 /Symbol findfont   43 sf 0    0 m 
(m)
 show 
 currentpoint pop 0 t 
 /Symbol findfont   30 sf 0  -14 m 
(I)
 show 
 currentpoint pop 0 t 
 /Helvetica-Bold findfont   43 sf 0    0 m 
( = 2 GeV\))
 show 
 gsave  gr  gr  595 850 210 136 C /w 9 def /w2 {w 2 div} def /w3 {w 3 div} def
 483 483 m5 1 lw 381 643 m -1 -3 d -1 -3 d -3 Y 1 -3 d 1 -4 d 2 -4 d 4 -9 d 3 -7
 d 2 -3 d 3 -10 d 5 -10 d 10 -20 d 9 -18 d 11 -21 d 14 -23 d 10 -17 d 15 -25 d 9
 -14 d 16 -24 d 11 -15 d 18 -26 d 11 -13 d 13 -16 d 3 -4 d 4 -4 d 10 -14 d 2 -2
 d 3 -2 d 2 X 2 1 d 1 1 d 1 1 d 2 4 d 1 2 d 1 3 d 1 3 d 3 Y -1 3 d -1 4 d -2 4 d
 -4 8 d -3 8 d -2 4 d -4 10 d -5 11 d -9 19 d -11 21 d -9 18 d -13 23 d -9 17 d
 -13 22 d -11 17 d -13 21 d -13 19 d -15 21 d -11 14 d -3 4 d -13 15 d -4 5 d -4
 4 d -10 13 d -2 3 d -3 1 d -4 X -2 -2 d -1 X -2 -4 d -2 -3 d -1 Y cl s 277 796
 m -2 -6 d -1 -5 d -6 Y 1 -6 d 2 -7 d 4 -10 d 8 -16 d 8 -15 d 3 -8 d 7 -18 d 10
 -22 d 21 -39 d 17 -33 d 27 -46 d 29 -49 d 18 -30 d 37 -58 d 14 -21 d 37 -55 d
 16 -24 d 37 -51 d 20 -28 d 26 -32 d 6 -7 d 7 -8 d 21 -31 d 4 -4 d 4 -2 d 4 X 3
 2 d 4 4 d 4 8 d 2 4 d 2 6 d 1 6 d 6 Y -1 7 d -2 7 d -4 10 d -8 16 d -7 14 d -3
 8 d -8 20 d -10 25 d -17 35 d -19 41 d -19 38 d -23 44 d -20 36 d -24 42 d -23
 37 d -24 38 d -28 42 d -28 38 d -22 28 d -11 13 d -24 28 d -11 11 d -9 10 d -20
 25 d -6 5 d -6 3 d -4 1 d -5 -1 d -4 -3 d -1 -1 d -6 -8 d -3 -5 d -1 -3 d cl s
 850 1020 0 0 C 595 850 210 136 C 850 1020 0 0 C
 gsave  492 519
 t   0 r 0 0 m
 /Symbol findfont   31 sf 0    0 m 
(t)
 show 
 gr  595 850 210 136 C 2 lw 370 536 m5 1 lw 329 545 m -1 Y 1 -2 d -2 Y 1 -2 d 1
 -2 d 1 -2 d 1 -2 d 1 -2 d 2 -2 d 2 -2 d 1 -1 d 2 -2 d 3 -2 d 2 -2 d 3 -2 d 1 X
 3 -2 d 3 -1 d 3 -1 d 2 -1 d 3 -1 d 3 X 2 -1 d 3 X 3 -1 d 12 X 2 1 d 2 X 2 1 d 3
 1 d 1 X 2 1 d 2 2 d 1 1 d 1 1 d 2 1 d 1 Y 1 2 d 1 1 d 2 Y 1 1 d 4 Y 1 1 d -1 2
 d 3 Y -1 2 d -1 2 d 2 Y -1 2 d -2 1 d -1 3 d -2 1 d -2 2 d -2 2 d -2 1 d -2 2 d
 -3 2 d -1 1 d -3 1 d -3 1 d -3 1 d -2 1 d -3 1 d -3 1 d -2 X -3 1 d -15 X -2 -1
 d -2 X -1 -1 d -3 X -2 -1 d -2 -1 d -2 -1 d -2 -1 d -1 -1 d -1 -2 d -1 X -1 -2
 d -1 -1 d -2 Y -1 -1 d -2 Y -1 -1 d -2 Y cl s 289 554 m -3 Y 1 -3 d -3 Y 2 -4 d
 2 -6 d 2 -3 d 2 -3 d 3 -4 d 4 -4 d 3 -4 d 4 -4 d 4 -3 d 5 -3 d 5 -4 d 6 -3 d 2
 -2 d 6 -2 d 6 -3 d 6 -2 d 4 -1 d 6 -2 d 7 -2 d 3 X 7 -2 d 6 X 5 -1 d 5 X 8 1 d
 5 X 5 1 d 4 1 d 2 1 d 5 1 d 3 2 d 4 1 d 1 Y 5 3 d 2 2 d 3 2 d 2 3 d 1 1 d 2 2 d
 1 4 d 2 3 d 1 4 d 1 3 d 11 Y -1 4 d -1 4 d -2 4 d -1 4 d -2 3 d -3 5 d -3 4 d
 -3 3 d -3 3 d -3 3 d -5 4 d -4 3 d -6 4 d -2 1 d -5 3 d -6 2 d -6 3 d -3 1 d -6
 2 d -6 1 d -4 1 d -6 1 d -6 1 d -17 X -7 -1 d -5 X -5 -1 d -2 -1 d -7 -2 d -4
 -1 d -4 -2 d -5 -3 d -4 -2 d -2 -2 d -2 -2 d -2 -1 d -2 -3 d -2 -3 d -2 -3 d -1
 -4 d -1 -3 d -1 -3 d -3 Y cl s 850 1020 0 0 C 595 850 210 136 C 850 1020 0 0 C
 gsave  344 462
 t   0 r 0 0 m
 /Helvetica-Bold findfont   31 sf 0    0 m 
(B)
 show 
 gr  595 850 210 136 C 2 lw 726 739 m5 1 lw 693 732 m -3 Y 1 -1 d -1 Y 1 -1 d 1
 X -1 Y 1 -1 d 2 -1 d 1 -1 d 2 X 1 -1 d 6 X 3 -1 d 3 X 2 1 d 5 X 3 1 d 2 X 2 1 d
 2 1 d 3 X 2 1 d 2 1 d 3 1 d 2 1 d 2 2 d 2 1 d 1 1 d 2 1 d 2 2 d 2 2 d 1 1 d 1 1
 d 1 2 d 1 2 d 1 Y 1 1 d 5 Y -1 2 d -1 1 d 1 Y -1 X -1 1 d -1 1 d -1 1 d -2 X -1
 1 d -3 X -2 1 d -8 X -3 -1 d -2 X -3 -1 d -3 X -1 -1 d -3 X -2 -1 d -3 -1 d -2
 -1 d -2 -1 d -2 -1 d -3 -1 d -2 -2 d -2 -1 d -1 -1 d -3 -2 d -1 -1 d -1 -2 d -1
 -1 d -1 -1 d -2 -2 d -2 Y -1 -1 d -2 Y cl s 659 725 m -2 Y 1 -3 d -2 Y 1 -2 d 2
 -2 d 1 -2 d 2 -1 d 1 -1 d 3 -2 d 4 -2 d 2 -1 d 4 -1 d 3 -1 d 3 -1 d 5 X 5 -1 d
 7 X 4 1 d 6 X 5 1 d 5 1 d 5 2 d 3 X 5 2 d 5 2 d 5 2 d 3 1 d 5 2 d 4 3 d 4 2 d 4
 3 d 4 2 d 3 2 d 4 5 d 3 3 d 3 2 d 1 2 d 2 3 d 2 4 d 2 3 d 3 Y 1 2 d 5 Y -1 3 d
 -1 2 d -1 2 d -1 2 d -2 2 d -2 1 d -2 2 d -2 1 d -3 1 d -2 1 d -3 1 d -3 X -4 1
 d -16 X -6 -1 d -4 X -6 -1 d -6 -2 d -2 X -6 -2 d -6 -2 d -5 -2 d -2 -1 d -6 -2
 d -4 -2 d -5 -3 d -5 -3 d -4 -2 d -2 -2 d -5 -4 d -4 -3 d -2 -2 d -2 -2 d -1 -2
 d -1 -1 d -2 -4 d -1 -3 d -1 -2 d -1 -2 d -3 Y cl s 850 1020 0 0 C 595 850 210
 136 C 850 1020 0 0 C
 gsave  720 674
 t   0 r 0 0 m
 /Symbol findfont   31 sf 0    0 m 
(r)
 show 
 gr  595 850 210 136 C 2 lw 641 493 m5 1 lw 601 490 m -2 Y 1 -1 d -1 Y 1 -1 d -1
 Y 1 -1 d 1 -1 d 1 -1 d 1 -1 d 2 X 2 -1 d 1 -1 d 3 -1 d 2 X 2 -1 d 3 -1 d 23 X 3
 1 d 1 X 3 1 d 3 X 2 1 d 2 1 d 3 1 d 2 1 d 3 1 d 2 1 d 1 1 d 1 1 d 3 2 d 1 1 d 1
 1 d 1 1 d 1 1 d 1 2 d 1 Y 1 1 d 5 Y -1 1 d -1 1 d 1 Y -1 1 d -1 1 d -1 X -1 1 d
 -1 1 d -1 1 d -2 X -2 1 d -2 1 d -3 X -3 1 d -2 X -3 1 d -11 X -4 -1 d -3 X -3
 -1 d -3 X -3 -1 d -3 -1 d -1 X -3 -1 d -3 -1 d -2 -1 d -2 -1 d -2 -1 d -1 -1 d
 -3 -2 d -1 -1 d -1 -1 d -1 -1 d -1 -1 d -1 -2 d -1 -1 d -1 Y -1 -1 d -1 Y cl s
 560 486 m -2 Y 1 -3 d 1 -2 d -1 Y 2 -2 d 1 -2 d 3 -3 d 3 -2 d 2 -1 d 3 -2 d 3
 -2 d 4 -1 d 5 -2 d 4 -1 d 5 -1 d 6 -2 d 5 X 6 -1 d 23 X 7 1 d 6 1 d 5 1 d 2 X 6
 1 d 6 2 d 5 1 d 3 1 d 5 2 d 5 3 d 5 2 d 3 2 d 4 2 d 1 1 d 4 4 d 4 2 d 2 3 d 2 2
 d 1 2 d 2 3 d 1 3 d 1 2 d 7 Y -1 2 d -1 3 d -1 2 d -1 2 d -2 2 d -2 2 d -2 2 d
 -3 1 d -3 2 d -3 2 d -4 1 d -4 1 d -4 1 d -7 1 d -4 1 d -6 1 d -21 X -7 -1 d -7
 -1 d -7 -1 d -7 -1 d -6 -1 d -6 -2 d -2 -1 d -6 -2 d -5 -2 d -4 -2 d -6 -2 d -4
 -2 d -2 -2 d -4 -2 d -4 -3 d -2 -2 d -2 -2 d -2 -2 d -1 Y -2 -2 d -1 -3 d -1 -2
 d -1 -2 d -3 Y cl s 850 1020 0 0 C 595 850 210 136 C 850 1020 0 0 C
 gsave  625 439
 t   0 r 0 0 m
 /Symbol findfont   31 sf 0    0 m 
(t)
 show 
 currentpoint pop 0 t 
 /Helvetica-Bold findfont   22 sf 0  -10 m 
(c)
 show 
 gr  595 850 210 136 C 2 lw 618 349 m5 1 lw 593 341 m -2 Y 1 X -1 Y 1 X -1 Y 3 X
 1 -1 d 6 X 2 1 d 4 X 2 1 d 1 X 2 1 d 2 1 d 3 X 1 1 d 2 1 d 2 1 d 2 1 d 2 1 d 1
 1 d 1 X 2 2 d 2 1 d 2 2 d 1 1 d 2 2 d 1 1 d 1 Y 1 1 d 1 Y -1 1 d 2 Y -1 X -1 1
 d -3 X -3 1 d -2 X -1 -1 d -4 X -2 -1 d -3 X -2 -1 d -2 -1 d -3 -1 d -1 X -2 -1
 d -2 -1 d -2 -1 d -2 -1 d -2 -1 d -1 -1 d -2 -1 d -1 -1 d -1 X -2 -2 d -1 Y -1
 X -2 -2 d -1 Y -1 -1 d -2 Y cl s 567 332 m -1 Y 1 -1 d 1 -2 d -1 Y 1 X 1 -1 d 1
 -1 d 2 X 1 -1 d 5 X 5 -1 d 5 X 3 1 d 4 X 3 1 d 4 X 4 2 d 2 X 4 1 d 5 2 d 4 1 d
 2 1 d 5 2 d 4 2 d 3 2 d 4 2 d 4 2 d 2 2 d 3 2 d 3 2 d 2 1 d 3 3 d 2 2 d 1 1 d 3
 4 d 1 2 d 1 1 d 3 Y 1 1 d -1 1 d 3 Y -1 1 d 1 Y -1 X -1 1 d -1 1 d -1 X -2 1 d
 -4 X -5 1 d -4 X -2 -1 d -4 X -4 -1 d -4 -1 d -4 -1 d -2 X -4 -2 d -5 -1 d -5
 -2 d -1 X -5 -2 d -4 -2 d -3 -2 d -4 -2 d -4 -2 d -2 -2 d -5 -2 d -3 -2 d -1 -1
 d -3 -3 d -2 -2 d -1 -1 d -4 -4 d -1 -2 d -1 -1 d -1 -1 d -4 Y cl s 850 1020 0
 0 C 595 850 210 136 C 850 1020 0 0 C
 gsave  605 295
 t   0 r 0 0 m
 /Helvetica-Bold findfont   31 sf 0    0 m 
(C)
 show 
 gr  595 850 210 136 C 850 1020 0 0 C
 gsave  357 935
 t   0 r 0 0 m
 /Helvetica-Bold findfont   43 sf 0    0 m 
(H1 Preliminary)
 show 
 gr 
 gsave  255 887
 t   0 r 0 0 m
 /Helvetica-Bold findfont   31 sf 0    0 m 
(Fits \260 la Dokshitzer, Webber et al.)
 show 
 gr 
 gsave  255 842
 t   0 r 0 0 m
 /Helvetica-Bold findfont   25 sf 0    0 m 
(1)
 show 
 currentpoint pop 0 t 
 /Symbol findfont   25 sf 0    0 m 
(s)
 show 
 currentpoint pop 0 t 
 /Helvetica-Bold findfont   25 sf 0    0 m 
(- and 2)
 show 
 currentpoint pop 0 t 
 /Symbol findfont   25 sf 0    0 m 
(s)
 show 
 currentpoint pop 0 t 
 /Helvetica-Bold findfont   25 sf 0    0 m 
(-contours \(stat. and exp. syst.\))
 show 
 gr 
 gsave  255 187
 t   0 r 0 0 m
 /Helvetica-Bold findfont   25 sf 0    0 m 
(pdf: MRSA'-115)
 show 
 gr 
 gr  gr 
showpage
end
%%EndDocument

